Holistically Explainable Vision Transformers

Transformers increasingly dominate the machine learning landscape across many tasks and domains, which increases the importance for understanding their outputs. While their attention modules provide partial insight into their inner workings, the attention scores have been shown to be insufficient for explaining the models as a whole. To address this, we propose B-cos transformers, which inherently provide holistic explanations for their decisions. Specifically, we formulate each model component - such as the multi-layer perceptrons, attention layers, and the tokenisation module - to be dynamic linear, which allows us to faithfully summarise the entire transformer via a single linear transform. We apply our proposed design to Vision Transformers (ViTs) and show that the resulting models, dubbed Bcos-ViTs, are highly interpretable and perform competitively to baseline ViTs on ImageNet. Code will be made available soon.

==> B-cos Transformers/0.1-abstract-v2.tex <==
Transformers increasingly dominate the machine learning landscape across many tasks and domains, which increases the importance for understanding their outputs. While their attention modules provide partial 
insight into their inner workings, the attention scores have been shown to be insufficient for explaining the models as a whole. 
To address this, we propose B-cos transformers, which inherently provide \emph{holistic} explanations for their decisions. 
Specifically, we formulate each model component---such as the multi-layer perceptrons, attention layers, and the  tokenisation module---to be \emph{dynamic linear}, which allows us to faithfully summarise the entire transformer via a single linear transform.
We apply our proposed design to Vision Transformers (ViTs) and
show that the resulting models, dubbed \textbf{Bcos-ViTs}, are highly interpretable and perform competitively to baseline ViTs on ImageNet.
Code will be made available soon.


==> B-cos Transformers/1-intro-v8.tex <==
\begin{wrapfigure}{b}{0.52\textwidth}
    \centering
    \vspace{-2em}
    \includegraphics[width=.51\textwidth]{resources/teaser2.pdf}\vspace{-.35em}
    \caption{Inherent explanations (cols.~2+3) of B-cos ViTs vs.\ attention explanations (cols.~4+5) for the same model. Note that $\mat W(\vec x)$ faithfully reflects the \emph{whole} model and yields more detailed and class-specific explanations than attention alone. For a detailed discussion, see supplement.}
    \label{fig:teaser}
    \vspace{-1em}
\end{wrapfigure}
Convolutional neural networks (CNNs) have dominated the last decade of computer vision. However, recently
they are often surpassed by 
transformers~\citep{vaswani2017attention}, which---if the current development is any indication---will replace CNNs for ever more tasks and domains.
Transformers are thus bound to impact many aspects of our lives: from healthcare, over judicial decisions, to autonomous driving. Given the sensitive nature of such areas, 
it is of utmost importance to ensure that we can explain the underlying models, which still remains a challenge for transformers. 

To explain transformers, prior work often 
focused on the models' attention layers~\citep{jain2019attention,serrano2019attention,abnar2020quantifying,barkan2021GradSAM}, as they inherently compute their output in an interpretable manner.
However, as transformers consist of many additional components, explanations derived from attention alone have been found insufficient to explain the full models~\citep{bastings2020,chefer2021transformer}. 
To address this, our goal is to develop transformers that inherently provide \emph{holistic} explanations for their decisions, i.e.\ explanations that reflect \emph{all} model components. 
These model components are given by: 
a {tokenisation} module, a mechanism for providing positional information to the model, multi-layer perceptrons (MLPs), as well as normalisation and attention layers, see~\cref{fig:sketch}a. 
By addressing the interpretability of each component individually, we obtain transformers that \emph{inherently} explain their decisions, see, for example \cref{fig:teaser} and \cref{fig:sketch}b.


In detail, our approach is based on the idea of designing each component to be 
\emph{dynamic linear}, such that it computes an input-dependent linear transform. This renders the entire model dynamic linear, cf.~\cite{Boehle2021CVPR,Boehle2022CVPR}, s.t.~it can be summarised by a single linear transform for each input.

In short, we make the following contributions. \colornum{(I)} We  present a novel approach for designing inherently interpretable transformers. For this,  \colornum{(II)} we carefully design each model component to be dynamic linear and ensure that their combination remains dynamic linear and interpretable.
Specifically, we address \colornum{(IIa)} the tokenisation module,  \colornum{(IIb)} the attention layers,  \colornum{(IIc)} the MLPs, and  \colornum{(IId)} the classification head.
 \colornum{(III)} Additionally, we introduce a novel mechanism for allowing the model to learn attention priors, which breaks the permutation invariance of transformers and thus allows the model to easily leverage positional information. In our experiments, we find that B-cos ViTs with such a learnt `attention prior' achieve significantly higher classification accuracies. 
  \colornum{(IV)} Finally, we evaluate a wide range of model configurations and show that the proposed B-cos ViTs are not only highly interpretable, but also constitute powerful image classifiers.

\begin{figure}[t]
    \centering\vspace{-1em}
    \begin{subfigure}[c]{0.435\textwidth}
    \includegraphics[height=11em, width=\textwidth]{resources/BcosViTs-Sketch3.pdf}
    \caption{}
    \label{fig:sketch1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[c]{0.545\textwidth}
    \vspace{.75em}
    \includegraphics[width=\textwidth, trim= 0 0 13em 0, clip]{resources/sketch3.pdf}
    \caption{}
    \label{fig:sketch2}
    \end{subfigure}
    \caption{
    \textbf{(a) B-cos ViTs.} We design each ViT component to be dynamic linear, allowing us to summarise the entire model by a single linear transform $\mat W(\vec x)$, as shown in the bottom. 
    \textbf{(b) Computation is Explanation.} 
    The model output is exactly computed by the linear transform $\mat W(\vec x)$. As a result, we can visualise this effective linear transform either by the corresponding matrix row (center) or the contributions $\vec c_k (\vec x)$ (right), cf.~\cref{eq:contribs}.
        }
    \label{fig:sketch}
    \vspace{-1.05em}
    
\end{figure}


==> B-cos Transformers/2-related-v2.tex <==
\myparagraph[0]{Attention as Explanation.} 
As the name exemplifies, attention is often thought to give insight into what a model `pays attention to' for its prediction. As such, various methods for using attention to understand the model output have been proposed, such as visualising the attention of single attention heads, cf.~\cite{vaswani2017attention}. However, especially in deeper layers the information becomes increasingly distributed and it is thus unclear whether a given token still represents its original position in the input~\citep{serrano2019attention,abnar2020quantifying}, thus complicating the interpretation of high attention values deep in the network~\citep{serrano2019attention,bastings2020}. 

Therefore, \cite{abnar2020quantifying} proposed  `attention rollout', which summarises the various attention maps throughout the layers. However, this summary still only includes the attention layers and neglects all other network components~\citep{bastings2020}. In response, various improvements over attention rollout have been proposed, such as GradSAM~\citep{barkan2021GradSAM} or an LRP-based explanation method~\citep{chefer2021transformer}, that were designed to more accurately reflect the computations of \emph{all} model components. The significant gains in quantitative interpretability metrics reported by \cite{chefer2021transformer} highlight the importance of such holistic explanations.


Similarly, we also aim to derive \emph{holistic} explanations for transformers. However, instead of deriving an explanation `post-hoc' as in \cite{chefer2021transformer}, we explicitly design our models to be holistically explainable. For this, we formulate each component---and thus the full model---to be dynamic linear.


\myparagraph{Dynamic Linearity.} Plain linear models, i.e.\ $y(\vec x) \myeq \mat w \vec x$, are usually considered interpretable, as $y(\vec x)$ can be  decomposed into individual contributions $c_i\myeq w_i\,x_i$ from any dimension $i$: $y \myeq \sum_i c_i$ \citep{melis2018towards}. However, linear models have a limited capacity, which has lead to various works aimed at extending their capacity without losing their interpretability, see \cite{melis2018towards,brendel2018approximating, Boehle2021CVPR, Boehle2022CVPR}. 
{An appealing} strategy for this is formulating \emph{dynamic} linear models~\citep{melis2018towards,Boehle2021CVPR,Boehle2022CVPR}, i.e.\ models that transform the input with a data-dependent matrix $\mat w(\vec x)$: $\vec y(\vec x)\myeq\mat w(\vec x)\vec x$. 

In this work, we rely on the B-cos framework \citep{Boehle2022CVPR}, but instead of focusing on CNNs as in \cite{Boehle2022CVPR}, we investigate the applicability of this framework to transformers. 


\myparagraph{Interpretability in DNNs.}
The question of interpretability extends, of course, beyond transformers and many methods for explaining DNNs have been proposed. 
While other approaches exist, cf.~\cite{kim2018tcav}, these methods typically estimate the importance of individual input features, which can be visualised as a heatmap, cf.~\cite{lundberg2017unified,petsiuk2018rise,ribeiro2016lime,simonyan2013deep,springenberg2014striving,zhou2016CAM,bach2015pixel,selvaraju2017grad,shrikumar2017deeplift,srinivas2019full,sundararajan2017axiomatic}.

Similarly, our models yield explanations in form of contribution heatmaps. However, in contrast to the above-referenced post-hoc explanation methods, the contribution maps of our B-cos ViTs are \emph{model-inherent}. Further, as the interpretability of the B-cos ViTs relies on aligning the weights with the inputs, the weights can be visualised in colour as in \cite{Boehle2022CVPR}, see \cref{fig:qualitative,,fig:teaser}.




==> B-cos Transformers/3-method-v5.tex <==
In the following, we present the overarching goal that we pursue and how we structure this section around it. First, however, we introduce the necessary background and the notation used in our work.

\textbf{Preliminaries.}
Vision Transformers (ViT) \citep{dosovitskiy2021an} with $L$ blocks are given by:
\begin{align}
    \label{eq:vit_def}
    \vec y (\vec x) = 
    \text{Classifier}\circ 
    \textstyle\prod_{l=1}^L \left(\text{MLPBlock}_l\circ \text{AttBlock}_l \right)\,\circ
    \text{Tokens}(\vec x)\, .
\end{align}
Here, the input $\vec x\in \mathbb R^{(CHW)}$ denotes a vectorised image of $H\myeq W$ height and width and with $C$ color channels; the functions, concatenated by $\circ$, 
are defined in Eqs.~\eqref{eq:bcostokens_def} - \eqref{eq:bcosclassifier_def} (left), with $\mat p,\mat e\in\mathbb R^{D\times N}$, $N$ the number of tokens and $D$ their dimensionality. 
%
Further, in Eqs.~\eqref{eq:bcostokens_def}~-~\eqref{eq:bcosclassifier_def}, 
CNN is a convolutional neural network\footnote{\label{foot:cnn}To simplify later equations, we take advantage of the fact that conv.~layers are equivalent to linear layers with weight constraints (weight sharing and local connectivity) and assume the CNN to process vectorised images.
},
$\mathcal T$ `tokenises' the CNN output (see \cref{subsec:backbone}),  Linear is a learnable linear transform $\vec{p'}(\vec p)\myeq\mat w\vec p\myplus\vec b$ with parameters $\mat w$ and $\vec b$ that is applied to each token $\vec p$ (columns of $\mat p$) independently, MSA denotes \underline{M}ulti-head \underline{S}elf-\underline{A}ttention, and $\mat E$ is a learnable embedding.
Following~\cite{graham2021levit}, Pool performs average pooling over the tokens, and the model output is given by $\vec y(\vec x)\in\mathbb R^{M}$ with $M$ classes.
Last, 
we omit indices for blocks and layers whenever unambiguous and it may be assumed that each layer has its own set of learnable parameters. 


\myparagraph{Our goal} in this work is to reformulate the ViTs such that they compute their output in a more interpretable manner. Specifically, we aim to make them \emph{dynamic linear} such that they compute
    $\vec y(\vec x) = \mat W (\vec x)\, \vec x $.
Instead of using the ViTs to predict $\mat W(\vec x)$, cf.~\cite{melis2018towards}, we achieve this by rendering each of the ViT components dynamic linear on their own  as follows:
\newcommand{\myarrow}{\;\;\highlight{\xrightarrow{\hphantom{\text{1234}
    }}}\;\;}
\boxalign{\begin{alignat}{8}
    % Tokens
    \label{eq:bcostokens_def}
    \text{Tokens} \,(&\vec x) &&=\; \mathcal T(\text{CNN}(\vec x)) + \mat E 
    &&\myarrow&&
    \text{\highlight{B-cos Tokens}}\, &&(\vec x) &&= \mat W^\text{Tokens}&&(\vec x)   &&  \;\vec x
    %
    %
    \\
    % Attention
    \label{eq:bcosatt_def}
    \text{AttBlock} \,(&\mat p) &&=\; \text{MSA}(\mat p) + \mat p
    &&\myarrow&&
    \text{\highlight{B-cos AttBlock}}\,&&(\mat p)  &&= \mat W^\text{Att} &&(\mat p)   &&  \;\mat p
    %
    %
    \\
    % MLP
    \label{eq:bcosmlp_def}
    \text{MLPBlock} \,(&\mat p) &&=\; \text{MLP}(\mat p) + \mat p 
    &&\myarrow&&
    \text{\highlight{B-cos MLPBlock}}\,&&(\mat p)  &&= \mat W^\text{MLP} &&(\mat p)   &&  \;\mat p
    %
    %
    \\
    % Classifier
    \label{eq:bcosclassifier_def}
    \text{Classifier}\, (&\mat p) &&=\; \text{Linear}\circ \text{Pool}(\mat p) 
    &&\myarrow&&
    \text{\highlight{B-cos Classifier}}\, &&(\mat P)
    &&= \mat W^\text{Class} &&(\mat p)   &&  \;\mat p
    \,.
\end{alignat}}
Crucially, we define each component such that it can be expressed as a dynamic linear function, see the right-hand side of Eqs.~\eqref{eq:bcostokens_def} - \eqref{eq:bcosclassifier_def}. 
As a result, the entire model will become dynamic linear:
\begin{align}
    \label{eq:bcosvit_def}
    \vec y (\vec x) = 
    \mat W^\text{Class}(\vec x)\; 
    \textstyle\prod_{l=1}^L \left(\mat W^\text{MLP}_l(\vec x) \; \mat W^\text{Att}_l(\vec x) \right)\,\;
    \mat W^\text{Tokens}(\vec x) \, \vec x=\mat w(\vec x)\,\vec x\,.
\end{align}
Specifically, we develop the B-cos ViTs in accordance with the B-cos framework~\citep{Boehle2022CVPR} to render $\mat w(\vec x)$ interpretable by aligning it with relevant input patterns.


\myparagraph[-.15]{Outline.} In the following, we shortly summarise the most relevant aspects of B-cos networks and
how to explain them (\cref{subsec:bcos}).
Then, we discuss 
Eqs.~\eqref{eq:bcostokens_def} - \eqref{eq:bcosclassifier_def} in detail and how we ensure that the resulting linear transform $\mat W(\vec x)$
will be interpretable.
In particular, we discuss the tokenisation (\cref{subsec:backbone}), attention (\cref{subsec:attention}), and the multi-layer perceptrons (\cref{subsec:mlps}). Finally, in \cref{subsec:pos_info}, we discuss how we encode positional information in B-cos ViTs, introducing `position-aware' attention.

\subsection{B-cos Networks: Interpretable Model-Inherent Explanations}
\label{subsec:bcos}




As shown in Eq.~\eqref{eq:bcosvit_def}, a dynamic linear transformer is summarised \emph{exactly} by a single matrix $\mat w(\vec x)$ for every $\vec x$. These linear explanations lend themselves well for understanding the model decisions: as in plain linear models, one can calculate linear contributions from individual features (e.g., pixels) to each output unit.
In detail, the effective linear contributions $\vec c_k$ to the $k$-th class logit are given by
\begin{align}
\label{eq:contribs}
\textbf{Dynamic Linear Contribution Maps:}\quad
    &\vec c_k(\vec x) = \left[\mat W(\vec x)\right]^T_k\odot \vec x\,,\quad\quad\quad
\end{align}
with $\odot$ denoting element-wise multiplication. Crucially, these contribution maps \emph{faithfully} summarise the entire model, as this linear summary is inherent to the model formulation, see also \cref{fig:sketch}. Thus, we use these {contribution maps} to explain the B-cos ViTs, see, e.g., \cref{fig:qualitative,,fig:teaser,,fig:sketch}. 


Note, however, that while the contribution maps in Eq.~\eqref{eq:contribs} accurately summarise any given dynamic linear model, this summary need not be \emph{interpretable}. E.g., for piece-wise linear models, which are also dynamic linear, 
this amounts 
to `Input$\times$Grad', cf.~\cite{adebayo2018sanity}.
For such models, however, the contributions $\vec c$ are very noisy and not easily interpretable for humans. Hence, we design the transformers in accordance with the `B-cos' framework~\citep{Boehle2022CVPR}, which ensures that $\mat w(\vec x)$ aligns with relevant input features and thus becomes easily interpretable.
In detail, the B-cos transform induces weight alignment by suppressing outputs for badly aligned weights:
\begin{align}
\label{eq:bcos}
    \text{B-cos} (\vec {a}; \mat w)  = 
    \left(\cos^{\text{B}-1}  (\vec a, \mat w) \odot  \widehat{\mat w} \right)\vec a = \mat w(\vec a)\vec a\;.
\end{align}
here, $\cos$ is applied row-wise, $\widehat{\mat w}$ denotes that the matrix rows are of unit norm, and $\odot$ represents row-wise scaling. As can be seen on the RHS of \cref{eq:bcos}, the B-cos transform is dynamic linear.

As a result, the matrix rows $[\mat W(\vec x)]_k$ align with relevant patterns of class $k$. 
By encoding the image such that the color is uniquely determined by the angle of the pixel encodings, it is possible to directly visualise those matrix rows in color, see \cref{fig:teaser,,fig:qualitative}. For details, see \cite{Boehle2022CVPR}.

\myparagraph{Requirements.} To ensure that a B-cos network aligns $\mat W(\vec x)$ with its inputs, each of its layers needs to \colornum{(a)} be bounded, \colornum{(b)} yield its maximum output if and only if its weight vectors align with its input, and \colornum{(c)} directly scale the overall \emph{model} output by its own output norm, see \cite{Boehle2022CVPR}. 
In the following, we ensure that each of the model components (Eqs.~\eqref{eq:bcostokens_def}-\eqref{eq:bcosclassifier_def}), fulfills these requirements. 



\subsection{Interpretable Tokenisation Modules: B-cos CNNs}
\label{subsec:backbone}
%
While the original Vision Transformer only applied a single-layered CNN, it has been shown that deeper CNN backbones yield better results and exhibit more stable training behaviour~\citep{xiao2021early}. 
%
Hence, to address the general case, and to take advantage of the increased training stability and performance, we take the tokenisation module to be given by a general CNN backbone. Being able to explain the \emph{full} ViT models consequently requires using an explainable CNN for this.

\myparagraph{Tokenisation.} We use B-cos CNNs~\citep{Boehle2022CVPR} as feature extractors; thus, the requirements \colornum{(a-c)}, \mbox{see \cref{subsec:bcos}, of B-cos networks are, of course, fulfilled. The input tokens are computed as}\\[-1.29em]
\boxalign{\begin{align}
    \text{B-cos Token}\; \vec p_i (\vec x) = \mathcal T_i \circ \text{B-cos CNN} (\vec x) = \highlight{\mat w^{\mathcal T_i}  \mat W^\text{CNN} (\vec x)} \, \vec x = \highlight{\mat W_i^\text{Tokens} (\vec x)}\, \vec x\,.
\end{align}
}
Here, $\vec p_i\myin\mathbb{R}^D$ corresponds to the $i$th column in the token matrix $\mat P$, $\mathcal T_i$ extracts the respective features from the CNNs' output with $\mat W^{\mathcal T_i}$ denoting the corresponding linear matrix. $\mat W^\text{CNN}$ is the dynamic linear mapping computed by the B-cos CNN, and as color-indicated, $\mat w_i^\text{Tokens}(\vec x)\myeq\mat W^{\mathcal T_i}\mat W^\text{CNN}(\vec x)$.


Finally, note that we did not include the additive positional embedding $\mat E$, cf.~\cref{eq:bcostokens_def} (left). For a detailed discussion on how to provide positional information to the B-cos ViTs, please see \cref{subsec:pos_info}.
\subsection{B-cos Attention}
\label{subsec:attention}
Interestingly, the attention operation itself is already dynamic linear and, as such, attention lends itself well to be integrated into the linear model summary according to Eq.~\eqref{eq:bcosvit_def}. 
To ensure that the resulting linear transformation maintains the desired interpretability, we discuss the necessary changes to make the attention layers compatible with the B-cos formulation as discussed in \cref{subsec:bcos}.




\myparagraph{B-cos Attention.} Note that conventional attention indeed computes a dynamic linear transform:
\begin{align}
\label{eq:attention}
    \text{Attention}({{\mat P}}; \mat Q,\mat K,\mat V) 
    \;&=\;
    \underbrace{\text{softmax}\left(\mat P^T\mat q^T {{\mat K}} {{\mat P}}\right)}_{\text{Attention matrix $\mat A({{\mat P}})$}}\underbrace{\,\mat v{{\mat P}}\,
    % Phantom to get underbrace on same height
    \vphantom{\text{softmax}\left(\mat q {{\mat P}} 
    {{\mat P}}^T\mat k^T\right)
    }
    % Phantom end
    }_{\text{Value}({\mat P})} 
    \;=\;
    \underbrace{\mat A({{\mat P}})\, \mat V
    % Phantom to get underbrace on same height
    \vphantom{\text{softmax}\left(\mat q {{\mat P}^T} 
    {{\mat P}}\mat k^T\right)
    }
    % Phantom end
    }_{\mat w({{\mat P}})}\, {{\mat P}}\; 
    \;=\; \mat W({{\mat P}}){{\mat P}}.
\end{align}
Here, $\mat q,\mat k$ and $\mat V$ denote the respective query, key, and value transformation matrices and $\mat P$ denotes the input tokens to the attention layer; further, softmax is computed column-wise.

In multi-head self-attention (MSA), see~\cref{eq:bcosatt_def} (left), $H$ distinct attention heads are used in parallel after normalising the input. Their concatenated outputs are then linearly projected by a matrix $\mat U$:
\begin{align}
    \text{MSA}(\widetilde{\mat P}) = \mat U \left[\mat W_1 (\widetilde{\mat P}) \widetilde{\mat P},\; \mat W_2 (\widetilde{\mat P}) \widetilde{\mat P},\; ...\;, \mat W_H (\widetilde{\mat P}) \widetilde{\mat P}\right] \quad \text{with}\quad \widetilde{\mat P} = \text{LayerNorm}(\mat P)
\end{align}

While this can still\footnote{To be exact, it can be represented as a dynamic \emph{affine} transform,  since LayerNorm adds a bias term.} be expressed as a dynamic linear transform of $\mat P$, we observe the following issues with respect to the requirements \colornum{(a-c)}, see \cref{subsec:bcos}. First, \colornum{(a)} while the attention matrix $\mat A({\mat P})$ is bounded, the value computation $\mat V{\mat P}$ and the projection by $\mat u$ are not. Therefore, as the output can arbitrarily increased by scaling $\mat V$ and $\mat u$, \colornum{(b)} a high weight alignment is not necessary to obtain large outputs.
Finally, by normalising the outputs of the previous layer, the scale of those outputs does not affect the scale of the overall model output anymore, which violates requirement \colornum{(c)}.

To address \colornum{(a+b)}, we propose to formulate a B-cos Attention Block as follows. First, we replace the value computation and the linear projection by $\mat u$ by corresponding B-cos transforms.
As in \cite{Boehle2022CVPR}, we employ MaxOut and for a given input $\mat P$ the resulting projections are computed as 
\begin{align}
    \label{eq:values}
    \text{B-cos Linear}({\mat P}; \mat S) 
    \;=\; \text{MaxOut} \circ \text{B-cos}(\mat P; \mat S)
    \;=\; 
    \mat W^{\mat s}(\mat P) \mat P \quad \text{with} \quad \mat S\in \{\mat U, \mat v\}.
\end{align}
To fulfill \colornum{(c)}, whilst not foregoing the benefits of LayerNorm\footnote{We noticed normalised inputs to be crucial for the computation of the attention matrix $\mat A({\mat P})$ in Eq.~\eqref{eq:attention}: for unconstrained inputs, softmax easily saturates and suffers from the vanishing gradient problem.}, we propose to exclusively apply LayerNorm before the computation of the attention matrix. i.e.\ we compute $\mat A(\mat P)$, see Eq.~\eqref{eq:attention} as 
\begin{align}
    \label{eq:normalisation}
    \mat A(\mat P; \mat Q, \mat K) = \text{softmax}\left( \widetilde{\mat P}^T\mat q^T \mat k\widetilde{\mat P}\right)
    \quad \text{with} \quad
    \widetilde{\mat P} = \text{LayerNorm}(\mat P)\,.
\end{align}
In total, a `B-cos AttBlock' thus computes the following linear transformation:
\boxalign{\begin{align}
\label{eq:bcosMSA_def}
    \text{B-cos AttBlock}({\mat P}) = 
    \highlight{
    \left(\mat W^{\mat u}(\mat P')
    \left[
        \mat A_h(\mat P) \mat W_h^{\mat V} (\mat P) \, 
    \right]_{h=1}^H + \mat I\right)}
    \mat P = \highlight{\mat W^\text{Att}(\mat p)} \; {\mat p}
    \;,
\end{align}}
Here, $\mat P' = \left[
        \mat A_h(\mat P) \mat W_h^{\mat V} (\mat P) \, 
    \right]_{h=1}^H$, $\mat W^{U}$  and $\mat W^{V}$ as in \cref{eq:values}, and $\mat A_h(\mat P)$ as in \cref{eq:normalisation}; the identity matrix $\mat I$ reflects the skip connection around the MSA computation, see~\cref{fig:sketch} and \cref{eq:bcosatt_def}.
    
    {For an ablation study regarding the proposed changes, we kindly refer the reader to the supplement.}

\subsection{Interpretable MLPs and Classifiers} 
\label{subsec:mlps}
To obtain dynamic linear and interpretable MLPs, we convert them to `B-cos' MLPs, such that they are compatible with the B-cos formulation (\cref{subsec:bcos}) and align their weights with relevant inputs.

\myparagraph{B-cos MLPs.} 
Typically, an MLP block in a ViT computes the following:
\begin{align}
    \text{MLPBlock}(\mat p) = \text{Linear}_2\circ \text{GELU}\circ \text{Linear}_1\circ \text{LayerNorm}(\mat p) + \mat p
\end{align}
Here, Linear is as in \cref{eq:bcosclassifier_def}, the GELU activation function is as in \cite{hendrycks2016gelu}, and LayerNorm as in~\cite{Ba2016LayerNorm}.

To obtain our `B-cos MLPBlock', we follow \cite{Boehle2022CVPR} and replace the linear layers by B-cos transforms, remove the non-linearities and the normalisation (cf.~\cref{subsec:attention}); further, each `neuron' is modelled by two units, to which we apply MaxOut~\citep{goodfellow2013maxout}.
As a result, each MLP block becomes dynamic linear:
\boxalign{\begin{align}
\label{eq:mlps}
    \text{B-cos MLPBlock}(\mat P)   
    &= \highlight{\left(
    \mat M_2 (\mat p)\, \mat l_2 (\mat p)\,
    \mat M_1 (\mat p)\, \mat l_1 (\mat p)
    + \mat I\right)}
    \mat p = \highlight{\mat W^\text{MLP}(\mat p)}\, \mat p\;.
\end{align}}
Here, $\mat M_i(\mat p)$ and $\mat l_i(\mat p)$ correspond to the effective linear transforms performed by the MaxOut and B-cos operation respectively, and $\mat I$ denotes the identity matrix stemming from the skip connection.

\myparagraph{Classifier.} Similar to the B-cos MLPs, we also replace the linear layer in the classifier, cf.~\cref{eq:bcosclassifier_def} (left), by a corresponding B-cos transform and the B-cos Classifier is thus defined as 
\boxalign{\begin{align}
    \text{B-cos Classifier}(\mat p) = \text{B-cos} \circ \text{Pool}(\mat P) = \highlight{\mat l(\mat P') \mat W^\text{AvgPool}}
    \mat P =\highlight{\mat W^\text{Class}(\mat P)}\, \mat p\;,
\end{align}}
with $\mat l(\mat P')$ the dynamic linear matrix corresponding to the B-cos transform and $\mat P'\myeq \text{Pool}(\mat P)$.



\subsection{Positional information in B-cos Transformers}
\label{subsec:pos_info}
In contrast to CNNs, which possess a strong inductive bias w.r.t.~spatial relations (local connectivity), transformers~\citep{vaswani2017attention} are invariant w.r.t.~the token order and thus lack such a `locality bias'. 
To nevertheless leverage spatial information, it is common practice to break the symmetry between tokens by adding a (learnt) embedding $\mat E$ to the input tokens $\mat P$, see \cref{eq:bcostokens_def} (left).

However, within the B-cos framework, this strategy is not optimal: 
in particular, note that each B-cos transformation needs to align its weights with its inputs to forward a large output to the next layer, see Eq.~\eqref{eq:bcos} and \cite{Boehle2022CVPR}. As a result, a {B-cos ViT} would need to associate contents (inputs) with specific positions, which could negatively impact the model's generalisation capabilities. 

Therefore, we investigate two alternative strategies for providing positional information to the B-cos ViTs: additive and multiplicative attention priors, see \cref{eq:addprior,eq:mulprior} respectively.
Specifically, we propose to add a learnable bias matrix $\mat B_h^l$ to each attention head $h$ in every layer $l$ in the model. This pair-wise (between tokens) bias is then either added\footnote{
Note that an additive positional bias in attention layers has been proposed before~\citep{graham2021levit}. 
} before the softmax operation or multiplied to the output of the softmax operation in the following way (omitting sub/superscripts):
%
{
\centering
\begin{minipage}{.415\textwidth}
\begin{align}
\label{eq:addprior}
 \mat A_\text{add}(\mat P) &= 
 \text{SM}\left(\mat R(\mat P) + \mat B\right)
\end{align}
\end{minipage}
\hfill
\begin{minipage}{.53\textwidth}
\begin{align}
 \label{eq:mulprior}
 \text{and}\quad\;
 \mat A_\text{mul}(\mat P) &=
 \text{SM}\left(\mat R(\mat P)\right)\times \text{SM}\left(\mat B\right)\;.
\end{align}
\end{minipage}
}\\[.5em]
Here, $\mat r(\mat P)\myeq \mat q \widetilde{\mat P} \widetilde{\mat P}^T\mat k^T$ and SM denotes softmax.
The bias $\mat b$ thus allows the model to learn an \emph{attention prior}, 
and the attention operation is no longer invariant to the token order. As such, the model can learn spatial relations between tokens and encode them explicitly in the bias matrix $\mat B$.
In our experiments, this significantly improved the performance of the B-cos ViTs, see \cref{subsec:results_acc}.

==> B-cos Transformers/4-experiments.tex <==
\myparagraph[0]{Dataset.} In this work, we focus on Vision Transformers (ViTs, \cite{dosovitskiy2021an}) for image classification. For this, we evaluate the B-cos and conventional ViTs and their explanations on the ImageNet dataset~\citep{deng2009imagenet}. We use images of size 224$\times$224. For B-cos models, we encode the images as in~\cite{Boehle2022CVPR}.

\myparagraph{Models.} We follow prior work and evaluate ViTs of different sizes in common configurations: Tiny (Ti), Small (S), and Base (B), cf.~\cite{steiner2021howtoVIT}. We train these models on the frozen features of publicly available~\citep{Boehle2022CVPR,torchvision} (B-cos) DenseNet-121 models and extract those features at different depths of the models: after 13, 38, or 87 layers. 
Model names are thus as follows: (B-cos) ViT-\{size\}-\{L\} with size$\in$\{Ti, S, B\} and L$\in$\{13, 38, 87\}.
We opted for (B-cos) DenseNet-121 backbones, as the conventional and the B-cos version achieve the same top-1 accuracy on the ImageNet validation set. 
%
In particular, we compare B-cos ViTs on B-cos backbones to normal ViTs on normal backbones.

\myparagraph{Training.} We employ a simple training paradigm that is common across models for comparability. 
All models are trained with RandAugment~\citep{cubuk2020randaugment} for 100 epochs with a learning rate of $2.5e^{-4}$, which is decreased by a factor of 10 after 60 epochs; for details, see supplement. 

\myparagraph{Evaluation Metrics.} We evaluate all models with respect to their accuracy on the ImageNet validation set. Further, we employ two common metrics to assess the quality of the model explanations.

First, we evaluate the grid pointing game~\citep{Boehle2021CVPR}. For this, we evaluate the explanations (see below) on 250 synthetic image grids of size 448$\times$448, containing 4 images of distinct classes, see Fig.~\ref{fig:localisation_sketch}; the individual images are ordered by confidence and we measure the fraction of positive attribution an explanation method assigns to the correct sub-image when explaining a given class. 

Note that, in contrast to fully convolutional networks, transformers with positional embeddings expect a fixed-size input. To nevertheless evaluate the models on such synthetic image grids, we scale down the image grid to the required input size of 224x224 to allow for applying the ViTs seamlessly.

Second, we evaluate two pixel perturbation metrics, cf.~\cite{chefer2021transformer}. For this, the pixels are ranked according to the importance assigned by a given explanation method. Then, we increasingly zero out up to 25\% of the pixels in increasing (decreasing) order, whilst measuring the model confidence in the ground truth class; a good explanation should obtain a high area under (over) the curve, i.e.\ the model should be insensitive to {unimportant} pixels and sensitive to important ones. 

We evaluate the perturbation metrics on the 250 most confidently and correctly classified images to enable a fair comparison between models, as the confidence affects the metrics; more details in supplement. Last, to succinctly summarise the two metrics, we evaluate the area \emph{between} the curves.

\myparagraph{Explanation Methods.} 
Apart from the model-inherent explanations (\cref{eq:contribs}), we evaluate two sets of explanation methods. 
First, we follow~\cite{chefer2021transformer} and evaluate common \emph{transformer-specific} explanations such as the attention in the final layer (FinAtt), attention rollout (Rollout)~\citep{abnar2020quantifying}, a transformer-specific LRP implementation (CheferLRP) proposed by \cite{chefer2021transformer}, `partial LRP'(pLRP)~\citep{voita2019analyzing}, and `GradSAM'~\citep{barkan2021GradSAM}. Further, we evaluate \emph{architecture-agnostic} methods such as Integrated Gradients (IntGrad)~\citep{sundararajan2017axiomatic}, adapted GradCAM~\citep{selvaraju2017grad} as in~\cite{chefer2021transformer}, and `Input$\times$Gradient' (IxG), cf.~\cite{adebayo2018sanity}. As no LRP rules are defined for B-cos ViTs we only apply it to baseline models. For method details, we kindly refer the reader to the supplement.

We evaluate all of those methods (if applicable) to the proposed B-cos ViTs, as well as the baselines consisting of conventional ViTs and backbones and compare them on the metrics described above. 


==> B-cos Transformers/5-results.tex <==
In the following, we present our experimental results.
%
Specifically, in \cref{subsec:results_acc} we analyse the classification performance of the B-cos ViTs: we investigate how the encoding of positional information affects model accuracy (see \cref{subsec:pos_info}) and compare the classification performance of B-cos and conventional ViTs.
%
Further, in \cref{subsec:results_explanations}, we evaluate the model-inherent explanations of the B-cos ViTs against common post-hoc explanation methods evaluated on the same models. To highlight the \emph{gain in interpretability} over conventional ViT models, we also compare the inherent explanations of the B-cos ViTs to the best post-hoc explanations evaluated on conventional ViTs, see supplement.


\subsection{Classification Performance of B-cos ViTs}
\label{subsec:results_acc}
\input{resources/figures/attention_ablation}
\input{resources/figures/accuracy_comparison}

In \cref{fig:attention_ablations}, we compare the top-1 ImageNet accuracy of various B-cos ViTs trained on the feature embeddings of the 87th layer of a frozen\footnote{
We chose to freeze the backbones to reduce the computational cost and compare the architectures across a wide range of settings. We observed comparable results when training the full models for individual architectures.

} B-cos DenseNet-121~\citep{Boehle2022CVPR}.
Specifically, we compare ViTs of different sizes (Tiny, Small, Base) and with different ways of allowing the models to use positional information, see \cref{eq:bcostokens_def,,eq:addprior,,eq:mulprior}.
We find that the multiplicative attention bias, see \cref{eq:mulprior}, consistently yields significant gains in performance. 
As discussed in \cref{subsec:pos_info}, we believe this could be due to the higher disentanglement between content and positional information. However, in preliminary experiments with \emph{conventional} ViTs, we did not observe significant benefits from such a multiplicative prior and this seems to be particularly advantageous for B-cos ViTs.

Interestingly, once trained with such a multiplicative attention prior, we find the B-cos ViTs to perform at least as good as their conventional counterparts over a wide range of configurations, see \cref{fig:accuracy_comparison}; {we find consistent results even without MaxOut in the Transformer layers (cf.~\cref{sec:method}), as we show in \cref{subsec:ablations2}.} However, these results have to be interpreted with caution: ViTs are known to be highly sensitive to, e.g., the amount of data augmentation, the number of training iterations, and model regularisation, see~\cite{steiner2021howtoVIT}. Moreover, our goal in this work is to develop interpretable ViTs and our focus thus lies on evaluating the quality of the explanations (\cref{subsec:results_explanations}).

\subsection{Interpretability of B-cos ViTs}
\label{subsec:results_explanations}
Here, we assess how well the inherent explanations (\cref{eq:contribs}) of B-cos ViTs explain their output and compare to common post-hoc explanations; {for comparisons to baseline ViTs, see supplement}.

\myparagraph{Localisation Metric.} In \cref{fig:loc_comp} (left), we plot the mean localisation score per model configuration (B-cos ViT-\{size\}-\{L\}) and explanation method, see \cref{sec:experiments}. 
We find that across all configurations, the model-inherent explanations according to \cref{eq:contribs} yield by far the best results under this metric and outperform the best \emph{post-hoc} explanation for the B-cos ViTs (Rollout) by a factor of $2.47$.

\input{resources/figures/combined_comparison}

\myparagraph{Pixel Perturbation.}
As for the localisation, in \cref{fig:loc_comp} (right), we plot the normalised mean area between the curves (ABC) per model configuration and explanation method of the B-cos ViTs. Specifically, the mean ABC is computed as the mean area between the curves when first removing the most / least important pixels from the images; we normalise the mean ABC for each explanation by the mean ABC of the model-inherent explanation (Ours) per model configuration to facilitate cross-model comparisons.
Again, the model-inherent explanations perform best and, on average, they outperform the second best post-hoc method (Rollout) on B-cos ViTs by a factor of $1.99$. 

\myparagraph{Qualitative Examples.} In \cref{fig:teaser,,fig:qualitative}, we qualitatively compare the inherent explanations (size: B, 38 backbone layers, see \cref{fig:accuracy_comparison}) to post-hoc explanations evaluated on the same model. As becomes apparent, the model-inherent summaries not only perform well quantitatively (cf.~\cref{fig:loc_comp}), but are also qualitatively convincing. Colour visualisations as in \cite{Boehle2022CVPR}; more results in supplement. In contrast to attention explanations, which are not class-specific~\citep{chefer2021transformer}, we find the model-inherent explanations of B-cos ViTs to be highly detailed and class-specific.
E.g., in \cref{fig:teaser}, we compare model-inherent explanations to attention-based explanations for single images from the ImageNet dataset which are inherently ambiguous. In \cref{fig:qualitative}, we evaluate the model on images as used in the localisation metric, see \cref{sec:experiments}, i.e.\ synthetic images with multiple classes. In both cases we find the model-inherent explanations to accurately highlight the respective features for the class logit that we aim to explain, whereas other methods are much less sensitive to the class logit; in fact, attention-based explanations are inherently agnostic to the choice of logit and thus the same for all classes.
For comparisons to explanations for
conventional ViTs, see the supplement.
%
\begin{figure}[t]
    \centering
    \includegraphics[width=1\textwidth]{resources/figures/comparison_example.pdf}
    \caption{
    Comparison of the model-inherent explanations (Ours) of a B-cos ViT-B-38, and several post-hoc explanations (GradSAM, GradCAM, Rollout, FinAtt, IntGrad) for class $k$ (left). 
    In particular, we show explanations for the classes `black swan', `forklift', `digital clock', and `lion' on a synthetic image containing these classes, as used in the localisation metric, see \cref{fig:localisation_sketch}. As B-cos ViTs follow the B-cos formulation, we can visualise the rows of $\mat W(\vec x)$ in colour~\citep{Boehle2022CVPR}. Additionally, we show contribution maps according to \cref{eq:contribs}. 
    }
    \vspace{-1.5em}
    \label{fig:qualitative}
\end{figure}

==> B-cos Transformers/6-discussion.tex <==
We present a novel approach for designing ViTs that are \emph{holistically} explainable. For this, we design every component of the ViTs with the explicit goal of being able to summarise the \emph{entire model} by a single linear transform. By integrating recent advances in designing interpretable dynamic linear models~\citep{Boehle2022CVPR}, these summaries become interpretable, as they are implicitly optimised to align with relevant input patterns. The resulting B-cos ViTs constitute competitive classifiers and their inherent linear summaries outperform any post-hoc explanation method on common metrics.

Compared to attention-based explanations, our method can be understood to `fill the blanks' in attention rollout~\citep{abnar2020quantifying}. Specifically, attention rollout computes a linear summary of the attention layers only. By integrating explanations for the remaining components (tokenisation, attention, MLPs), we are able to obtain \emph{holistic} explanations of high detail, see \cref{fig:teaser,,fig:qualitative}.

As transformers are highly modality-agnostic, we believe that our work has the potential to positively impact model interpretability across a wide range of domains. Evaluating B-cos transformers on different tasks and modalities is thus an exciting direction that we aim to explore in future work.

\myparagraph{Limitations.}
While the B-cos ViTs allow us to extract model-faithful explanations for single images, note that these explanations are always \emph{local} in nature, i.e.\ for single data points. The explanations thus help understanding an \emph{individual} classification, but do not directly give insights into which features the models most focus on over the \emph{entire dataset}. It would thus be interesting to combine B-cos ViTs with \emph{global} explanation methods, such as in \cite{bau2017network,kim2018tcav}.

Further, we focused primarily on the designing of interpretable transformers, and, to test across a wide range of models, limited experiments to the ImageNet-1k dataset. As transformers are known to significantly benefit from additional data and training~\citep{dosovitskiy2021an}, it would be interesting to test the limits of capacity of the B-cos ViTs and scale to more complex tasks.






==> B-cos Transformers/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> B-cos Transformers/packages_and_commands.tex <==
\usepackage{iclr2023_conference}
\usepackage{times}
\usepackage{natbib}
\iclrfinalcopy
\usepackage[export]{adjustbox}
\usepackage{booktabs}
\usepackage{times}
\usepackage{epsfig}
\usepackage{ifthen}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{amssymb}
\usepackage{subcaption}
\usepackage{wrapfig}
\usepackage{multirow}
\usepackage{parskip}
\usepackage{array}
\usepackage{xr-hyper}
\usepackage{enumitem}       % enumerations
\usepackage{caption}
\captionsetup{font=small}
\usepackage{xcolor}
\usepackage{todonotes}
\usepackage{changepage}
\usepackage[hang,flushmargin]{footmisc} 
\usepackage[pagebackref,breaklinks,colorlinks]{hyperref}
\definecolor{ForestGreen}{RGB}{56, 176, 0}
\hypersetup{
    colorlinks,
    linkcolor={red},
    citecolor={ForestGreen},
    urlcolor={blue}
}
\usepackage{tikz}
\newcommand{\boxalign}[2][0.97\textwidth]{
 \noindent\tikzstyle{mybox} = [draw=black,inner sep=6pt, thick]
 \begin{center}\vspace{-.75em}\begin{tikzpicture}
  \node [mybox] (box){%
   \begin{minipage}{#1}{\vspace{-3mm}#2}\end{minipage}
  };
 \end{tikzpicture}\end{center}
}

\setlength{\parskip}{5pt minus 1pt}


\usepackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\Crefname{table}{Table}{Tables}
\crefname{table}{Tab.}{Tabs.}
\renewcommand{\figurename}{Fig.}
\renewcommand{\tablename}{Tab.}
% Equal sign with less space
\newcommand\myeq{\mkern1.25mu{=}\mkern1.25mu}
\newcommand\myminus{\mkern1.25mu{-}\mkern1.25mu}
\newcommand\myplus{\mkern1.25mu{+}\mkern1.25mu}
\newcommand\mygreater{\mkern1.25mu{>}\mkern1.25mu}
\newcommand\myin{\mkern1.25mu{\in}\mkern1.25mu}
\newcommand\mytimes{\mkern1.25mu{\times}\mkern1.25mu}
\newcommand\mysubsub[1]{\vspace{-.7em}%
\subsubsection{#1}%
\vspace{-.6em}
}
\newcommand\mysub[1]{\subsection{#1}}

% Result tables
\newcolumntype{R}[2]{%
    >{\adjustbox{angle=#1,lap=\width-(#2)}\bgroup}%
    l%
    <{\egroup}%
}
\newcommand*\rot{\multicolumn{1}{R{90}{1em}}}
\makeatletter
\def\thickhline{%
  \noalign{\ifnum0=`}\fi\hrule \@height \thickarrayrulewidth \futurelet
   \reserved@a\@xthickhline}
\def\@xthickhline{\ifx\reserved@a\thickhline
               \vskip\doublerulesep
               \vskip-\thickarrayrulewidth
             \fi
      \ifnum0=`{\fi}}
\makeatother

\newlength{\thickarrayrulewidth}
\setlength{\thickarrayrulewidth}{3.5\arrayrulewidth}


%%%%%%%%%%%%%%
%% COMMANDS %%
%%%%%%%%%%%%%%
\DeclareMathOperator{\sign}{sign}
\newcommand{\colornum}[1]{{\textbf{\color[RGB]{39, 158, 206}#1}}}
\newcommand{\highlight}[1]{{{\color[RGB]{39, 158, 206}#1}}}
\newcommand{\mat}[1]{\MakeUppercase{\mathbf{#1}}}
\renewcommand{\vec}[1]{\MakeLowercase{\mathbf{#1}}}
\newcommand{\tmat}[1]{$\mat{#1}$}
\newcommand{\tvec}[1]{$\vec{#1}$}
\newcommand{\boldit}[1]{\textbf{\textit{#1}}}
\newcommand{\bcos}{B-cos}
\newcommand{\mbcos}{\text{B-cos}}
\newcommand{\upd}[1]{
{%\color[rgb]{0, 0.5, 0.5}
#1}
}
\newcommand{\rebuttal}[1]{
{%\color[rgb]{0, 0.5, 0.5}
#1}
}

\newboolean{showcomments}
\setboolean{showcomments}{false}
\newcommand{\showappendix}{\input{7-appendix}}

\newcommand{\myparagraph}[2][.1]{\vspace{#1em}\noindent{\bf #2}}


==> B-cos Transformers/resources/figures/accuracy_ablation.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[c]{\textwidth}
    \includegraphics[height=14em, width=\textwidth]{resources/accuracy_ablations/maxout_comparison.pdf}
    \caption{Comparison between B-cos ViTs with (solid) and without (striped) MaxOut in the Transformer layers.
    }
    \end{subfigure}
    \begin{subfigure}[c]{\textwidth}
    \includegraphics[height=14em, width=\textwidth]{resources/accuracy_ablations/maxout_comparison2bline.pdf}
    \caption{Comparison between B-cos ViTs (no MaxOut) (striped) in the Transformer layers and conventional ViTs.}
    \end{subfigure}
    \caption{
    \textbf{Understanding the impact of MaxOut on model performance.} 
    \textbf{(a)} For the Tiny transformers, we find that MaxOut indeed significantly improves model performance. However, this performance gap between models with and without MaxOut closes with increasing model size (Small and Base). \textbf{(b)}
    As such, when comparing to conventional ViTs (same numbers as in \cref{fig:accuracy_comparison}), we find that B-cos ViTs without MaxOut can achieve similar performance without adding additional parameters in the Transformer layers, as long as the initial model size is sufficiently large.
    }
    \label{fig:accuracy_ablation}
\end{figure}


==> B-cos Transformers/resources/figures/accuracy_comparison.tex <==
\begin{figure}
    \centering
    \includegraphics[height=14em, width=\textwidth]{resources/accuracy_ablations/bline_comparison.pdf}
    \caption{
    ImageNet accuracies of B-cos ViTs with a multiplicative attention bias (Eq.~\eqref{eq:mulprior}) compared to standard ViTs and backbones, both for differently sized ViTs (Tiny, Small, Base) and backbones (13, 38, or 87 layers). 
    We find that the B-cos ViTs perform at least as well as the baseline ViTs over almost all tested configurations.
    }
    \label{fig:accuracy_comparison}
\end{figure}


==> B-cos Transformers/resources/figures/attention_ablation.tex <==

\begin{figure}
\begin{minipage}[c]{0.58\linewidth}
\begin{minipage}[c][4.75cm]{\linewidth}
\includegraphics[height=12em]{resources/accuracy_ablations/attention_version.pdf}
\end{minipage}
\caption{ImageNet accuracy of differently sized B-cos ViTs (Tiny, Small, Base) depending on the positional encoding.
We find B-cos ViTs with $\mat A_\text{mul}$, see  Eq.~\eqref{eq:mulprior}, to perform significantly better.
}
\label{fig:attention_ablations}
\end{minipage}
\hfill
\begin{minipage}[c]{0.4\textwidth}
\begin{minipage}[c][4.75cm]{\linewidth}
\includegraphics[height=12em]{resources/Localisation_example.pdf}
\end{minipage}%
\caption{In the localisation metric, we measure the fraction of pos.~evidence assigned to the correct grid cell for each occurring class.
}
\label{fig:localisation_sketch}
\end{minipage}\vspace{-.5em}
\end{figure}



% \begin{figure}
%     \centering
    
%     \caption{
%     ImageNet top-1 accuracy of differently sized transformers (Tiny, Small, Base) depending on how positional information is encoded (\textbf{left}), see Sec.~\ref{subsec:pos_info}, and the size of the backbone model (\textbf{right}).
%     We find that product attention (see Eq.~\eqref{eq:mulprior}) improves model performance (left plot). Further, the model accuracy improves with the size of the transformer model (left and right plots) and with the size of the backbone model (right plot).
%     }
%     \label{fig:attention_ablations}
% \end{figure}

==> B-cos Transformers/resources/figures/combined_comparison.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{resources/localisation/combined_comparison2.pdf}
    \caption{ 
    Quantitative comparison of explanation methods according to two metrics: localisation (\textbf{left}) and perturbation (\textbf{right}); for a description of metrics and methods, see \cref{sec:experiments}.
    We evaluated the methods for all B-cos ViTs shown in \cref{fig:accuracy_comparison} and plot the corresponding scores (markers). We also plot the mean score over all models (dashed lines) per method and the average improvement of the \emph{model-inherent} over the best \emph{post-hoc} explanation (localisation:$\,\times2.47$, perturbation:$\,\times1.99$). Note that for the perturbation metric, we normalised the area between curves (ABC) by the scores of the model-inherent explanations for better cross-model comparison.
    }
    \label{fig:loc_comp}
    \vspace{-1em}
\end{figure}

==> B-cos Transformers/resources/figures/combined_metrics.tex <==
\begin{figure}
\begin{minipage}[t]{1\linewidth}
\input{resources/figures/localisation_comparison}
\input{resources/figures/perturbation_comparison}
\end{minipage}
\end{figure}

==> B-cos Transformers/resources/figures/interpretability-localisation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{resources/localisation/inter-acc.pdf}
    \caption{
    ImageNet top-1 accuracy of differently sized transformers (Tiny, Small, Base) depending on how positional information is encoded (\textbf{left}), see Sec.~\ref{subsec:pos_info}, and the size of the backbone model (\textbf{right}).
    We find that product attention (see Eq.~\eqref{eq:mulprior}) improves model performance (left plot). Further, the model accuracy improves with the size of the transformer model (left and right plots) and with the size of the backbone model (right plot).
    }
    \label{fig:attention_ablations}
\end{figure}

==> B-cos Transformers/resources/figures/localisation_comparison.tex <==
%\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{resources/localisation/loc_comparison.pdf}
    \caption{ \mario{could be helpful to start the legend with "explaination method:" ... if there is space}
    \textbf{Localisation scores} of various explanation methods evaluated on B-cos \textbf{(left)} and conventional ViTs \textbf{(right)} (one score per model). We further plot the mean across models per method (dashed lines). We find the linear summaries of B-cos ViTs, cf.~\cref{eq:contribs}, to perform best, beating attention rollout by $\Delta\myeq0.71$ on average. Further, they score significantly higher than the state-of-the-art methods on conventional ViTs ($\Delta\myeq0.34$). \bernt{does the reader get to know what GradSAM, Rollout, etc is? I would suggest to add references in the figure or the caption -- in the text we need a bit of argumentation why we are using those for comparison -- at the moment that seems entirely arbitrary I'd say}
    }
    \label{fig:loc_comp}
%\end{figure}

==> B-cos Transformers/resources/figures/perturbation_comparison.tex <==
%\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{resources/pixel_removal/pert_comparison.pdf}
    \caption{
    \textbf{Area between pixel removal curves} of various explanations evaluated on B-cos \textbf{(left)} and conventional ViTs \textbf{(right)}. As in \cref{fig:loc_comp}, we additionally show the mean across models per method (dashed lines). We find the linear summaries of B-cos ViTs, cf.~\cref{eq:collapse}, to consistently rank best, beating attention rollout by $\Delta\myeq\ 0.06$ on average. Further, they score significantly higher than the best methods for conventional ViTs ($\Delta\myeq\ 0.05$). \bernt{this plots seems far less convincing than fig 5 -- also the right side looks rather confusing as the points are all of the place for the different methods -- clear candidate to move to the supplement imo}
    }
    \label{fig:pixel_removal}
%\end{figure}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> resources/figures/combined_metrics.tex <==
\begin{figure}
\begin{minipage}[t]{1\linewidth}
\input{resources/figures/localisation_comparison}
\input{resources/figures/perturbation_comparison}
\end{minipage}
\end{figure}

==> resources/figures/interpretability-localisation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{resources/localisation/inter-acc.pdf}
    \caption{
    ImageNet top-1 accuracy of differently sized transformers (Tiny, Small, Base) depending on how positional information is encoded (\textbf{left}), see Sec.~\ref{subsec:pos_info}, and the size of the backbone model (\textbf{right}).
    We find that product attention (see Eq.~\eqref{eq:mulprior}) improves model performance (left plot). Further, the model accuracy improves with the size of the transformer model (left and right plots) and with the size of the backbone model (right plot).
    }
    \label{fig:attention_ablations}
\end{figure}

==> resources/figures/localisation_comparison.tex <==
%\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{resources/localisation/loc_comparison.pdf}
    \caption{ \mario{could be helpful to start the legend with "explaination method:" ... if there is space}
    \textbf{Localisation scores} of various explanation methods evaluated on B-cos \textbf{(left)} and conventional ViTs \textbf{(right)} (one score per model). We further plot the mean across models per method (dashed lines). We find the linear summaries of B-cos ViTs, cf.~\cref{eq:contribs}, to perform best, beating attention rollout by $\Delta\myeq0.71$ on average. Further, they score significantly higher than the state-of-the-art methods on conventional ViTs ($\Delta\myeq0.34$). \bernt{does the reader get to know what GradSAM, Rollout, etc is? I would suggest to add references in the figure or the caption -- in the text we need a bit of argumentation why we are using those for comparison -- at the moment that seems entirely arbitrary I'd say}
    }
    \label{fig:loc_comp}
%\end{figure}

==> resources/figures/perturbation_comparison.tex <==
%\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{resources/pixel_removal/pert_comparison.pdf}
    \caption{
    \textbf{Area between pixel removal curves} of various explanations evaluated on B-cos \textbf{(left)} and conventional ViTs \textbf{(right)}. As in \cref{fig:loc_comp}, we additionally show the mean across models per method (dashed lines). We find the linear summaries of B-cos ViTs, cf.~\cref{eq:collapse}, to consistently rank best, beating attention rollout by $\Delta\myeq\ 0.06$ on average. Further, they score significantly higher than the best methods for conventional ViTs ($\Delta\myeq\ 0.05$). \bernt{this plots seems far less convincing than fig 5 -- also the right side looks rather confusing as the points are all of the place for the different methods -- clear candidate to move to the supplement imo}
    }
    \label{fig:pixel_removal}
%\end{figure}

